Offline Task Assistance Planning on a Graph:Theoretic and Algorithmic Foundations

In this work we introduce the problem of task assistance planning where we are given two robots Rtask and Rassist. The first robot, Rtask, is in charge of performing a given task by executing a precomputed path. The second robot, Rassist, is in charge of assisting the task performed by Rtask using on-board sensors. The ability of Rassist to provide assistance to Rtask depends on the locations of both robots. Since Rtask is moving along its path, Rassist may also need to move to provide as much assistance as possible. The problem we study is how to compute a path for Rassist so as to maximize the portion of Rtask's path for which assistance is provided. We limit the problem to the setting where Rassist moves on a roadmap which is a graph embedded in its configuration space and show that this problem is NP-hard. Fortunately, we show that when Rassist moves on a given path, and all we have to do is compute the times at which Rassist should move from one configuration to the following one, we can solve the problem optimally in polynomial time. Together with carefully-crafted upper bounds, this polynomial-time algorithm is integrated into a Branch and Bound-based algorithm that can compute optimal solutions to the problem outperforming baselines by several orders of magnitude. We demonstrate our work empirically in simulated scenarios containing both planar manipulators and UR robots as well as in the lab on real robots.

==> sections/Hardness_new.tex <==
\section{Hardness of the OPTP Problem}
\label{sec:hardness}

We now move on to the OPTP problem and show that it is $\NP$-hard.
Roughly speaking, the hardness of the problem comes from the fact that in the general setting, there may be an exponential number of paths in a graph and in contrast to the shortest-path problem, Bellman’s principle of optimality does not hold. 
%
%For example, in many cases, adding a  vertex to a path will not improve the reward even if that vertex contains intervals from which the task can be assisted, but adding that same vertex and one of its neighbors might significantly improve the reward. \os{can we generate a simple example to depict this?}


\begin{thm}
    \label{thm:hardness}
    The OPTP problem is $\NP$-hard.
\end{thm}

\begin{proof}[Sketch]
    The proof is by a reduction from the subset-sum problem (SSP)~\cite{kleinberg2006algorithm}.
    Recall that the SSP is a decision problem where we are given 
    a set 
    $X = \{x_1, \dots, x_n \mid~x_i \in \mathbb{N} \}$
    and a target 
    $\k \in \mathbb{N}^{+}$\conference{}{(for simplicity, we assume that $\k>0$ but this is a technicality only)}. 
    The problem calls for deciding whether there exists a set $X' \subseteq X$ whose sum $\sum_{x\in X'} x$~equals $K$.

    Given an SSP instance, we build a corresponding OPTP instance (to be explained shortly) and show that there exists a subset $X' \subseteq X$ such that $\sum_{x\in X'} x = \k$ iff the optimal reward in our OPTP instance is $\frac{\k}{\sum_{i=1}^{n}{x_i}} + 1$ thus proving the problem is $\NP$-hard.
    
    W.l.o.g. assume that 
    $x_1, \dots, x_n$ are sorted from smallest to largest
    and set
    $\kappa_i:= \sum_{j=1}^{i} x_j$,
    $\alpha_i := x_i / \kappa_n$ and $y_i = \sum_{j=1}^{i-1}{\kappa_j}$. 
    %
    The graph of our OPTP instance depicted in Fig.~\ref{fig:reduction} contains 
    $n$ hexagons $H_1, \ldots H_n$ such that $H_i$ contains vertices~$a_i, b_i, c_i, d_i, e_i, f_i$. 
    We call $a_i$ and $f_i$ the entry and exit vertices of $H_i$,
    $b_i$ and $c_i$ the top of $H_i$
    and
    $d_i$ and $e_i$ the bottom of $H_i$.
    %
    Edges $(b_i,c_i)$ and $(d_i,e_i)$ at the top and bottom of $H_i$ have length $\kappa_i$ and $\kappa_{i-1}$, respectively (all other edge lengths are equal to zero).
    Edge $(b_i,c_i)$ at the top of $H_i$ contains the interval $[y_i, y_i + \alpha_i]$.\footnote{Strictly speaking, the interval belongs to the vertices $b_i, c_i$. However, it will be more convenient to consider the interval as belonging to the edge $(b_i,c_i)$.} 
    %
    Finally, the exit $f_n$ of the last hexagon $H_n$ has an edge to a vertex~$v$ whose interval is $[y_n + \k, y_n + \k + 1]$.
    Note that here for ease of exposition, time is in the range $[0, y_n+\k+1]$ and \emph{not}  $[0,1]$. 
    

\begin{figure}[tb]
    \centering
    \includegraphics[scale=1]{new_reduction_final}
    \caption{
        Reduction graph (all edges are directed from left to right). 
        When omitted, edge length equals zero.
    }
    \label{fig:reduction}
    \vspace{-5mm}
\end{figure}

     Our reduction is based on three key properties of the new OPTP instance:
    \begin{itemize}
        \item [P1]
        Every optimal path must reach $v$.
        \item[P2]
        The shortest path to reach $v$ is by taking the lower part of each $H_i$ and its length is $y_n$.
        \item[P3] 
        Let $\pi$ be a path that reaches $v$.
        Going through the upper part of~$H_i$ adds additional $x_i$ time to reach $u$ and results in an additional reward of~$\alpha_i$.
    \end{itemize}

    %\EB{Read again}
    Roughly speaking, the interval at~$v$ forces any path $\pi$ to reach $v$ at time $y_n + \k$ (Property~$P1$). 
    %
    As the minimal time to reach $u$ is $y_n$ (Property~$P2$),~$\pi$ only has $\k$ time units to spend on earning rewards from the hexagons.
    %
    Now, to obtain a reward of $\k/\kappa_n + 1$, $\pi$ must earn a reward of $\k/\kappa_n$ before reaching~$u$.
    %
    Since the upper part of $H_i$ adds an additional time of $x_i$ and a reward of $\alpha_i$ (Property~$P2$),~$\pi$ must find a combination of upper parts $I_{\text{up}}$ such that $\sum_{i \in I_{\text{up}}}{x_i} = \k$ which is the exact solution to the subset-sum problem.
\end{proof}



